PyTorch Geometric Temporal: Spatiotemporal Signal Processing with Neural Machine Learning Models

We present PyTorch Geometric Temporal a deep learning framework combining state-of-the-art machine learning algorithms for neural spatiotemporal signal processing. The main goal of the library is to make temporal geometric deep learning available for researchers and machine learning practitioners in a unified easy-to-use framework. PyTorch Geometric Temporal was created with foundations on existing libraries in the PyTorch eco-system, streamlined neural network layer definitions, temporal snapshot generators for batching, and integrated benchmark datasets. These features are illustrated with a tutorial-like case study. Experiments demonstrate the predictive performance of the models implemented in the library on real world problems such as epidemiological forecasting, ridehail demand prediction and web-traffic management. Our sensitivity analysis of runtime shows that the framework can potentially operate on web-scale datasets with rich temporal features and spatial structure.

==> code_snippets/model_definition_2.tex <==
\begin{code}


\begin{minted}[linenos,fontsize=\small,xleftmargin=0.5cm,numbersep=3pt,frame=lines]{python}
import torch
import torch.nn.functional as F
from torch_geometric_temporal.nn.recurrent import DCRNN

class RecurrentGCN(torch.nn.Module):
    def __init__(self, node_features, filters):
        super(RecurrentGCN, self).__init__()
        self.recurrent = DCRNN(node_features, filters, 1)
        self.linear = torch.nn.Linear(filters, 1)

    def forward(self, x, edge_index, edge_weight):
        h = self.recurrent(x, edge_index, edge_weight)
        h = F.relu(h)
        h = F.dropout(h, training=self.training)
        h = self.linear(h)
        return h
\end{minted}
\captionof{listing}{Defining a recurrent graph convolutonal neural network using PyTorch Geometric Temporal consisting of a diffusion convolutional spatiotemporal layer followed by rectified linear unit activations, dropout and a feedforward neural network layer.}\label{code:model_definition}
\end{code}

==> code_snippets/temporal_split_2.tex <==
\begin{code}
\begin{minted}[linenos,fontsize=\small,xleftmargin=0.5cm,numbersep=3pt,frame=lines]{python}
from torch_geometric_temporal import ChickenpoxDatasetLoader
from torch_geometric_temporal import temporal_signal_split

loader = ChickenpoxDatasetLoader()

dataset = loader.get_dataset()

train, test = temporal_signal_split(dataset,
                                    train_ratio=0.9)
\end{minted}
\captionof{listing}{Loading a default benchmark dataset and creating a temporal split with PyTorch Geometric Temporal}\label{code:split_example}
\end{code}
